Rethinking the Evaluation for Conversational Recommendation in the Era of Large Language Models

The recent success of large language models (LLMs) has shown great potential to develop more powerful conversational recommender systems (CRSs), which rely on natural language conversations to satisfy user needs. In this paper, we embark on an investigation into the utilization of ChatGPT for conversational recommendation, revealing the inadequacy of the existing evaluation protocol. It might over-emphasize the matching with the ground-truth items or utterances generated by human annotators, while neglecting the interactive nature of being a capable CRS. To overcome the limitation, we further propose an interactive Evaluation approach based on LLMs named iEvaLM that harnesses LLM-based user simulators. Our evaluation approach can simulate various interaction scenarios between users and systems. Through the experiments on two publicly available CRS datasets, we demonstrate notable improvements compared to the prevailing evaluation protocol. Furthermore, we emphasize the evaluation of explainability, and ChatGPT showcases persuasive explanation generation for its recommendations. Our study contributes to a deeper comprehension of the untapped potential of LLMs for CRSs and provides a more flexible and easy-to-use evaluation framework for future research endeavors. The codes and data are publicly available at https://github.com/RUCAIBox/iEvaLM-CRS.

==> section/related_work.tex <==
\section{Related Work}

In this section, we summarize the related work from the following perspectives.

\subsection{Conversational Recommender System}

The fields of conversation intelligence~\cite{gao2018neural} and recommendation systems~\cite{wu2022survey} have seen significant progress in recent years. 
One promising development is the integration of these two fields, leading to the emergence of conversational recommender systems~(CRSs)~\cite{jannach2021survey, gao2021advances}. 
CRSs provide recommendations to users through conversational interactions, which has the potential to significantly improve the user experience.

One popular approach~\cite{lei2020estimation, tu2022conversational} assumes that interactions with users primarily take the form of question answering, where users are asked about their preferences for items and their attributes. The goal is to learn an optimal interaction strategy that captures user preferences and provides accurate recommendations in as few turns as possible. However, this approach often relies on hand-crafted templates and does not explicitly model the language aspect of CRSs.
% CRSs in this category are usually system-driven, \ie they proactively seek to acquire user preference by asking questions.
Another approach~\cite{zhang2023variational, zhou-etal-2022-aligning} focuses on engaging users in more free-form natural language conversations, such as chit-chat. The aim is to capture user preferences from the conversation context and generate recommendations using persuasive responses.

Our work belongs to the second category.
In this work, we systematically evaluate the performance of large language models~(LLMs) like \chatgpt for conversational recommendation on large-scale datasets.
% Most of the CRSs in this line of work are user-driven, \ie they can only make recommendations passively according to the conversation history with users.
% Although various external data (\eg knowledge graphs~\cite{} and item reviews~\cite{}) and techniques (\eg graph neural networks~\cite{} and pre-trained language models~\cite{}) have been utilized, user-driven CRSs still face the problem of ambiguous user preference in limited conversation context.
% The first line of work can resolve this issue to some extent by proactively asking questions to users about their preferences, however, the proposed questions are restricted to pre-defined templates~\cite{}, which greatly limits their applications.

% In this work, we consider two kinds of conversations, \ie attribute-based question answering and free-form chit-chat, to comprehensively evaluate the performance of \chatgpt for conversational recommendation through proactive preference elicitation.
% The results show that \chatgpt can perform better under the setting of chit-chat based conversation than attribute-based conversation on specific datasets.

\subsection{Language Models for Conversational Recommendation}

There have been recent studies on how to integrate language models~(LMs) into CRSs.
One notable investigation by~\citet{penha2020does} evaluates the performance of the pre-trained language model~(PLM) BERT~\cite{kenton2019bert} in conversational recommendation.
% They manually design several prompt templates to probe the knowledge stored in BERT and find that it has more content-based knowledge than collaborative-based knowledge.
% To resolve this, the authors propose to infuse both kinds of knowledge via multitask fine-tuning for improving performance.
Other studies~\cite{wang2022towards, yang2022improving, deng2023unified, friedman2023leveraging} primarily utilize PLMs as the foundation to build unified CRSs, capable of performing various tasks using a single model instead of multiple components.
PLMs can also be utilized for synthesizing CRS datasets~\cite{lu2023august, guo2023towards, qu2023towards}.
% Inspired by the generalizability of PLMs for solving various tasks, some recent studies utilize them as the backbones to develop unified CRSs, which can solve various subtasks using just one model instead of multiple components.
% \citet{} develop a unified CRS through fine-tuning PLMs on specific datasets.
% They expand the vocabulary of PLMs with an extra item vocabulary, and utilize the pointer mechanism to control the switch between target item and general token generation.
% Other studies use the recently proposed paradigm prompting~\cite{} to further unify the subtasks of CRSs.
% \citet{} append a special token \texttt{[REC]} to the conversation history as the prompt to summarize the context information for recommendation.
% \citet{} extent this and design specific prompts for each subtask of CRSs to fine-tune PLMs with prompt-based multitask learning.
% In contrast, \citet{} fix the PLMs and only fine-tune the task-specific prompts to inject the knowledge required for different subtasks.
However, the current approaches are mainly confined to small-size LMs like BERT~\cite{kenton2019bert} and DialoGPT~\cite{zhang2020dialogpt}.

In this paper, we focus on the evaluation of CRSs developed with not only PLMs but also LLMs and propose a new evaluation approach \methodname.

\subsection{Evaluation and User Simulation}

The evaluation of CRSs remains an area that has not been thoroughly explored in existing literature.
Previous studies have primarily focused on turn-level evaluation~\cite{li2018towards, chen2019towards}, where the system output of a single turn is compared against ground-truth labels for two major tasks: conversation and recommendation.
Some researchers have also adopted conversation-level evaluation to assess conversation strategies~\cite{lei2020estimation, zhang2018towards, balog2023user}.
In such cases, user simulation is often employed as a substitute for human evaluation.
These approaches typically involve collecting real user interaction history~\cite{lei2020estimation} or reviews~\cite{zhang2018towards} to represent the preferences of simulated users.
However, due to the intricate and interactive nature of conversational recommendation, the evaluation is often constrained by pre-defined conversation flows or template-based utterances. Consequently, this limitation hinders the comprehensive assessment of the practical utility of CRSs.

In our work, we propose an interactive evaluation approach \methodname with LLM-based user simulators, which has a strong instruction-following ability and can flexibly adapt to different CRSs based on the instruction without further tuning.
